Multi-Objective $\textit{min-max}$ Online Convex Optimization

In this paper, we broaden the horizon of online convex optimization (OCO), and consider multi-objective OCO, where there are $K$ distinct loss function sequences, and an algorithm has to choose its action at time $t$, before the $K$ loss functions at time $t$ are revealed. To capture the tradeoff between tracking the $K$ different sequences, we consider the {\it min-max} regret, where the benchmark (optimal offline algorithm) takes a static action across all time slots that minimizes the maximum of the total loss (summed across time slots) incurred by each of the $K$ sequences. An online algorithm is allowed to change its action across time slots, and its {\it min-max} regret is defined as the difference between its {\it min-max} cost and that of the benchmark. The {\it min-max} regret is a stringent performance measure and an algorithm with small regret needs to `track' all loss functions simultaneously. We first show that with adversarial input, {\it min-max} regret scales linearly with the time horizon $T$ for any online algorithm. Consequently, we consider a stochastic i.i.d. input model where all loss functions are i.i.d. generated from an unknown joint distribution and propose a simple algorithm that combines the well-known {\it Hedge} and online gradient descent (OGD) and show via a remarkably simple proof that its expected {\it min-max} regret is $O(\sqrt{T \log (T K)})$. Analogous results are also derived for Martingale difference and Markov input models.

==> AdaptivePrediction.tex <==
\section{With Predictions}
\begin{algorithm}[H]
\caption{Minimization of the Maximum of Two Convex Losses}
\label{alg:main}
\begin{algorithmic}[1]
\State \textbf{Input:} step sizes $\eta_{x,t} > 0$, $\eta_{\theta,t} > 0$
\State \textbf{Initialize:} $w_1 = (1,1)$, $\theta_1 = w_1 / \|w_1\|_1$, $f_0\equiv 0, g_0\equiv 0$ and pick arbitrary $x_0 \in \mathcal{X}$
\For{$t=1,\dots,T$}

  \State Observe $\lambda_{t-1}(x_{t-1}) = (f_{t-1}(x_{t-1}),g_{t-1}(x_{t-1}))$ and $\Lambda_{t-1}(x_{t-1},\theta_t)$ using current $\theta_t$
  \State Get predicted ${\tilde \lambda}_t(x_{t-1})= ({\tilde f}_{t}(x_{t-1}),{\tilde g}_{t}(x_{t-1}))$ and ${\tilde \Lambda}_{t}(x_{t-1},\theta_t)$ using current $\theta_t$
 % true gradient  $\Lambda_t(x_{t-1},\theta_t)$ and predicted gradient ${\tilde \Lambda}_{t}(x_{t-1},\theta_t)$
  \State Cumulative Gradient Error $E_{x,t} \gets E_{x,t-1} + \|\Lambda_{t-1}(x_{t-1},\theta_t) - {\tilde \Lambda}_{t-1}(x_{t-1},\theta_t)\|_\infty^2$
  \State $\eta_{x,t} \gets \dfrac{\eta_{x,0}}{\sqrt{E_{x,t}}}$
  \State Play $x_t = \textbf{Optimistic AdaGrad}(\eta_{x,t}, x_{t-1}, {\tilde \Lambda}_{t}(x_{t-1},\theta_t), \Lambda_{t-1}(x_{t-1},\theta_t))$ 
   \State Cumulative Loss Error $E_{\theta, t} \gets E_{\theta, t-1} + \|\lambda_{t-1}(x_{t-1}) - \tilde \lambda_{t-1}(x_{t-1})\|_\infty^2$
    \State $\eta_{\theta, t} \gets \dfrac{\eta_0}{\sqrt{E_{\theta, t}}}$
  \State {\bf Hedge:} $w_{t+1} = \textbf{Optimistic AdaHedge}
  (\eta_{\theta, t}, w_{t,i}, {\tilde \lambda}_t(x_{t-1}), \lambda_{t-1}(x_{t-1}))$
  \State Normalize: $\theta_{t+1} = w_{t+1}/\|w_{t+1}\|_1$
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{Optimistic AdaGrad $(\eta, x, {\tilde h}, h)$}
\label{alg:optimistic-adagrad}
\begin{algorithmic}[1]
\Require Convex set $\mathcal{K} \subset \mathbb{R}^d$, 
%\State Initialize $G_0 \gets \delta >0$
%\For{$t=1,\dots,T$}
    %\State $G_t \gets G_{t-1} + \|\lambda_t - \tilde \lambda_t\|^2$
    %\State $\eta_t \gets \dfrac{\eta_0}{\sqrt{G_t}}$
    \State $y \gets \Pi_{\mathcal{K}}\!\left(x - \eta \tilde h\right)$
    \State Return $z \gets \Pi_{\mathcal{K}}\!\left(y - \eta h\right)$
%\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{Optimistic AdaHedge $(\eta, w_t,  {\tilde \lambda}, \lambda, )$}
\label{alg:optimistic-adahedge}
\begin{algorithmic}[1]
%\Require Number of experts $N$, initial weights $w_1(i)=\frac{1}{N}$, $\eta_0>0$
%\State Initialize $G_0 \gets \delta>0$
%\For{$t=1,\dots,T$}
   % \State Receive predicted loss vector $\tilde \ell_t \in \mathbb{R}^N$
    \State $\hat w_t(i) \propto w_t(i) \exp\!\left( \eta_t \tilde \lambda(i) \right)$
   % \State Normalize $\hat w_t$
    %\State Play according to $\hat w_t$
    \State Return $w_{t+1}(i) \propto \hat w_t(i) \exp\!\left( \eta_t \left(\lambda(i) - {\tilde \lambda}(i)\right) \right)$
%\EndFor
\end{algorithmic}
\end{algorithm}



\section{Optimistic Adaptive Hedge — Gains Version}

Let \(\lambda_t \in [0,1]^N\) be the gain vector at time \(t\), and \({\tilde \lambda}_t \in [0,1]^N\) be the predicted gain vector.  
Let \(\eta_t > 0\) be the learning rate and \(\theta_t \in \Delta_N\) the normalized weight vector.  
Let the regularizer be the negative entropy:
\[
R(u) = \sum_{i=1}^N u(i) \log u(i).
\]
The Bregman divergence is the KL divergence:
\[
D_R(u \,\|\, v) 
= D_{\mathrm{KL}}(u \,\|\, v) 
= \sum_{i=1}^N u(i) \log\frac{u(i)}{v(i)}.
\]


\subsection*{KL Divergence Bound}
\begin{lemma}
From the update rule and the properties of the exponential weights, we have:
\begin{align}
D_R(\theta_t \,\|\, \theta_{t-1})
&= \eta_t \langle {\tilde \lambda}_t, \theta_t \rangle 
- \log Z_t \nonumber \\
&\le -\eta_t 
\langle \lambda_t - {\tilde \lambda}_t, \theta_t - \theta_{t-1} \rangle 
+ \frac{\eta_t^2}{2} 
\|\lambda_t - {\tilde \lambda}_t\|_\infty^2.
\label{eq:kl-bound}
\end{align}

\end{lemma}
\begin{proof}
\subsection*{Derivation of the KL Bound}

Recall the two-step update for \(\theta_t\):

\textbf{Step 1: Prediction Step}
\[
\tilde{\theta}_{t}(i) 
= \frac{\theta_{t-1}(i) 
e^{\eta_t \tilde{\lambda}_t(i)}}{ 
\sum_{j=1}^N 
\theta_{t-1}(j) e^{\eta_t \tilde{\lambda}_t(j)} },
\]
with normalization constant
\[
Z_t 
:= \sum_{j=1}^N 
\theta_{t-1}(j) e^{\eta_t \tilde{\lambda}_t(j)}.
\]

\textbf{Step 2: Correction Step}
\[
\theta_{t}(i) 
= \frac{\tilde{\theta}_{t}(i) 
e^{\eta_t \left( \lambda_t(i) 
- \tilde{\lambda}_t(i) \right)}}
{ \sum_{j=1}^N 
\tilde{\theta}_{t}(j) 
e^{\eta_t \left( \lambda_t(j) 
- \tilde{\lambda}_t(j) \right)} }.
\]
Let \(\tilde{Z}_t\) denote this normalization constant.

Substituting \(\tilde{\theta}_t(i)\) from Step 1 into Step 2:
\[
\theta_t(i) 
= \frac{\theta_{t-1}(i) 
e^{\eta_t \tilde{\lambda}_t(i)} 
e^{\eta_t \left( \lambda_t(i) 
- \tilde{\lambda}_t(i) \right)}}
{Z_t \,\tilde{Z}_t} 
= \frac{\theta_{t-1}(i) 
e^{\eta_t \lambda_t(i)}}
{Z_t \,\tilde{Z}_t}.
\]

Thus the update is an exponential-weights update with gain vector \(\lambda_t\) and normalization \(Z_t \tilde{Z}_t\):
\[
\theta_t(i) 
= \frac{\theta_{t-1}(i) 
e^{\eta_t \lambda_t(i)}}{Z'_t}, 
\quad Z'_t := Z_t \tilde{Z}_t.
\]

By definition of KL divergence for negative entropy regularization:
\[
D_R(\theta_t \,\|\, \theta_{t-1}) 
= \sum_{i=1}^N 
\theta_t(i) 
\log \frac{\theta_t(i)}{\theta_{t-1}(i)} 
= \eta_t \langle \lambda_t, \theta_t \rangle 
- \log Z'_t.
\]

From Step 1 and Step 2 we have:
\[
Z'_t 
= \sum_{j=1}^N 
\theta_{t-1}(j) 
e^{\eta_t \lambda_t(j)},
\]
which yields:
\[
D_R(\theta_t \,\|\, \theta_{t-1}) 
= \eta_t \langle \lambda_t, \theta_t \rangle 
- \log \sum_{j=1}^N 
\theta_{t-1}(j) 
e^{\eta_t \lambda_t(j)}.
\]

\begin{proposition}\label{prop:kl}
\[
D_R(\theta_t \,\|\, \theta_{t-1})
\;\le\;
\eta_t
\langle \lambda_t - \tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
+
\eta_t
\langle \tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
+
\frac{\eta_t^2}{2}
\|\lambda_t - \tilde{\lambda}_t\|_\infty^2.
\]
\end{proposition}
\begin{proof}
\subsection*{Proof of Step 1: Bound on $D_R(\theta_t \,\|\, \theta_{t-1})$ via $Z_t$ expansion}

Recall that
\begin{equation}\label{eq:dummy2}
D_R(\theta_t \,\|\, \theta_{t-1})
= \eta_t\sum_{i=1}^n
\theta_t(i)\tilde{\lambda}_t(i) - \log Z_t,
\end{equation}
where
\[
Z_t
= \sum_{j=1}^n
\theta_{t-1}(j)\exp\!\left(\eta_t\tilde{\lambda}_t(j)\right).
\]

Since $\log$ is concave, using Jensen’s inequality:
\[
\log Z_t
\ge
\eta_t
\sum_{j=1}^n
\theta_{t-1}(j)\tilde{\lambda}_t(j).
\]

Also, by a second‑order expansion (smoothness of the exponential):
\[
\log Z_t
\le
\eta_t
\sum_{j=1}^n
\theta_{t-1}(j)\tilde{\lambda}_t(j)
+ \frac{\eta_t^2}{2}
\|\tilde{\lambda}_t\|_\infty^2.
\]

Using these lower and upper bounds in \eqref{eq:dummy2}, we get 
\[
D_R(\theta_t \,\|\, \theta_{t-1})
\le
\eta_t
\sum_{i=1}^n
\theta_t(i)\tilde{\lambda}_t(i)
- \eta_t
\sum_{j=1}^n
\theta_{t-1}(j)\tilde{\lambda}_t(j)
+ \frac{\eta_t^2}{2}
\|\tilde{\lambda}_t\|_\infty^2.
\]

Rewriting, we get
\begin{equation}\label{eq:dummy3}
D_R(\theta_t \,\|\, \theta_{t-1})
\le
\eta_t
\langle
\tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
+ \frac{\eta_t^2}{2}
\|\tilde{\lambda}_t\|_\infty^2.
\end{equation}





To make the expression dependent on the prediction error, we write
\[
\lambda_t = \tilde{\lambda}_t + (\lambda_t - \tilde{\lambda}_t).
\]
which implies that
\[
\langle
\tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
= \langle
\lambda_t,
\theta_t - \theta_{t-1}
\rangle
- \langle
\lambda_t - \tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle.
\]
Substituting this in \eqref{eq:dummy3}, we get the 
\[
D_R(\theta_t \,\|\, \theta_{t-1})
\le
\eta_t
\langle
\lambda_t,
\theta_t - \theta_{t-1}
\rangle
- \eta_t
\langle
\lambda_t - \tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
+ \frac{\eta_t^2}{2}
\|\lambda_t - \tilde{\lambda}_t\|_\infty^2.
\]


\end{proof}


\begin{theorem}[Total movement bound for Adaptive Optimistic Hedge]
Let $\theta_t$ be the normalized weights produced by Adaptive Optimistic Hedge (gains version), with bounded gains:
\[
\|\lambda_t\|_\infty \le c,\quad
\|\tilde{\lambda}_t\|_\infty \le c,
\]
and define the prediction error:
\[
\mathrm{error}_t := \|\lambda_t - \tilde{\lambda}_t\|_\infty.
\]
Let the step-size be
\[
\eta_t := \frac{1}{\sqrt{1 + \sum_{s=1}^{t-1} \mathrm{error}_s^2}}.
\]
Then there exists a constant $C>0$ such that:
\[
\boxed{
\sum_{t=1}^T
\|\theta_t - \theta_{t-1}\|_1
\;\le\;
C\sqrt{1 + \sum_{t=1}^T \mathrm{error}_t^2}
\left(
1 + \sqrt{\log T}
\right).
}
\]
\end{theorem}

\begin{proof}
From Proposition \ref{prop:kl}, 
\[
D_R(\theta_t \,\|\, \theta_{t-1})
\;\le\;
\eta_t
\langle \lambda_t - \tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
+
\eta_t
\langle \tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
+
\frac{\eta_t^2}{2}
\|\lambda_t - \tilde{\lambda}_t\|_\infty^2.
\]
By H\"older's inequality:
\[
\langle \lambda_t - \tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
\le
\mathrm{error}_t
\|\theta_t - \theta_{t-1}\|_1,\quad
\langle \tilde{\lambda}_t,
\theta_t - \theta_{t-1}
\rangle
\le
c
\|\theta_t - \theta_{t-1}\|_1.
\]
Thus:
\[
D_R(\theta_t \,\|\, \theta_{t-1})
\le
\eta_t
\left(
c + \mathrm{error}_t
\right)
\|\theta_t - \theta_{t-1}\|_1
+
\frac{\eta_t^2}{2}
\mathrm{error}_t^2.
\]

Applying Pinsker's inequality:
\[
\|\theta_t - \theta_{t-1}\|_1^2
\le
2 D_R(\theta_t \,\|\, \theta_{t-1}),
\]
we get:
\[
\|\theta_t - \theta_{t-1}\|_1^2
\le
2\eta_t
\left(
c + \mathrm{error}_t
\right)
\|\theta_t - \theta_{t-1}\|_1
+
\eta_t^2
\mathrm{error}_t^2.
\]

Let $x_t := \|\theta_t - \theta_{t-1}\|_1$ and $a_t := 2\eta_t(c + \mathrm{error}_t)$, $b_t := \eta_t^2\mathrm{error}_t^2$.  
We have:
\[
x_t^2 - a_t x_t - b_t \le 0.
\]
Thus:
\[
x_t \le \frac{a_t + \sqrt{a_t^2 + 4b_t}}{2}
\le a_t + \sqrt{b_t}.
\]
Therefore:
\[
\|\theta_t - \theta_{t-1}\|_1
\le
2\eta_t(c + \mathrm{error}_t)
+
\eta_t\mathrm{error}_t
\le
C \eta_t\left(
1 + \mathrm{error}_t
\right),
\]
for some constant $C>0$ depending on $c$.

Summing over $t$:
\[
\sum_{t=1}^T
\|\theta_t - \theta_{t-1}\|_1
\le
C
\sum_{t=1}^T
\eta_t
+
C
\sum_{t=1}^T
\eta_t \,\mathrm{error}_t.
\]

For adaptive $\eta_t = \frac{1}{\sqrt{1 + \sum_{s=1}^{t-1}\mathrm{error}_s^2}}$:
\[
\sum_{t=1}^T \eta_t
\le
2\sqrt{1 + \sum_{t=1}^T \mathrm{error}_t^2}.
\]
Also:
\[
\sum_{t=1}^T
\eta_t\,\mathrm{error}_t
\le
\sqrt{
\sum_{t=1}^T
\eta_t^2
}
\sqrt{
\sum_{t=1}^T
\mathrm{error}_t^2
}.
\]
But:
\[
\sum_{t=1}^T
\eta_t^2
=
\sum_{t=1}^T
\frac{1}{1 + \sum_{s=1}^{t-1}
\mathrm{error}_s^2}
\le
\log\!\left(
1 + \sum_{t=1}^T
\mathrm{error}_t^2
\right),
\]
by telescoping.  
Hence:
\[
\sum_{t=1}^T
\eta_t\,\mathrm{error}_t
\le
\sqrt{
\sum_{t=1}^T
\mathrm{error}_t^2
}
\sqrt{
\log\!\left(
1 + \sum_{t=1}^T
\mathrm{error}_t^2
\right)
}.
\]

Combining:
\[
\sum_{t=1}^T
\|\theta_t - \theta_{t-1}\|_1
\le
C
\sqrt{1 + \sum_{t=1}^T
\mathrm{error}_t^2}
\left(
1 + \sqrt{
\log\!\left(
1 + \sum_{t=1}^T
\mathrm{error}_t^2
\right)
}
\right).
\]
Since $\log(1+x) \le \log T$ for $x\le T$, this yields:
\[
\boxed{
\sum_{t=1}^T
\|\theta_t - \theta_{t-1}\|_1
\le
C
\sqrt{1 + \sum_{t=1}^T
\mathrm{error}_t^2}
\left(
1 + \sqrt{\log T}
\right).
}
\]
\end{proof}




==> BinaryCase.tex <==
\section{Binary Sequences}
In this section, we consider the special case when sequences $f_t^k \in \{0,1\}$ are binary sequences for all $k=1,\dots, K$. The setup is as before, an online algorithm $\cA$ has 
to choose a binary action $x_t\in\{0,1\}$ before $f_t^k$'s are revealed at time $t$ and incurs a loss 
\begin{equation}\label{defn:costbit}
C_\cA = \max_{k=1, \dots, K}\left\{\sum_{t=1}^T \mathbf{1}\{x_t \ne f_t^{(k)}\}\right\},
\end{equation}
while the cost of $\opt$ that chooses a single action $x$ is 
\begin{equation}
C_\opt = \min_{x\in\{0,1\}} \max_{k=1,\dots,K} \sum_{t=1}^T \mathbf{1}\{x \ne f_t^{(k)}\}.
\end{equation}
Consequently, the regret is 
\begin{equation}
R_\cA (T) = \sup_{f_t^k} \{C_\cA - C_\opt\}.
\end{equation}


When $K=1$, this is a very well studied problem called {\it universal prediction of binary sequences} \cite{feder2002universal, cover1966behavior}, and for which it is known that Follow-the-Leader (FTL) algorithm achieves constant regret when 
the input is i.i.d. \cite{feder2002universal}, while Cover's algorithm \cite{cover1966behavior} achieves a $O(\sqrt{T})$ regret with the worst-case input. Compared to Section \ref{sec:iid}, where we could 
show a sub-linear regret guarantee only when the input was i.i.d., in this simplified binary input case, we will propose an algorithm call \textsf{BIT} that has regret $O(\sqrt{T})$  even when the input is worst-case.

The basic idea of \textsf{BIT} is to consider a surrogate function $\ell_t(p)  =\max_{k=1,\dots,K}\; |p - f_t^{k}|$ and then execute OGD (using sub-gradients) with respect to $\ell_t(p)$ to choose the probability $p$ with which $x_t=1$ is played. To derive the regret guarantee, we use the OGD regret result with respect to the surrogate function $\ell_t(p),$ and then connect that to the true cost of \textsf{BIT} \eqref{defn:costbit}.

\begin{algorithm}[H]
\caption{\textsf{BIT}}
\label{alg:prob-ogd-K}
\begin{algorithmic}[1]
\Require  Step-size $\eta>0$ and  initialize $p_1=1/2$)
\For{$t=1,\dots,T$}
  \State Sample $x_t\sim\mathrm{Bernoulli}(p_t)$ and play $x_t$.
  \State Observe the \(K\) bits $(f_t^{1},\dots,f_t^{K})\in\{0,1\}^K$.
  \State Define the convex surrogate loss
    \[
      \ell_t(p) \;:=\; \max_{k=1,\dots,K}\; |p - f_t^{k}|,\qquad p\in[0,1].
    \]
  \State Choose any subgradient $s_t\in\partial\ell_t(p_t)$ (note $|s_t|\le 1$).
  \State Gradient step and projection:
    \[
      y_{t+1} \leftarrow p_t - \eta s_t,\qquad
      p_{t+1} \leftarrow \text{Proj}_{[0,1]}(y_{t+1}).
    \]
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{theorem}


With $\eta=1/\sqrt{T}$, Algorithm \textsc{BIT} satisfies
\[
\quad
\mathbb{E}\{R_{\textsf{BIT}}(T)\}  \le O(\sqrt{KT}).
\quad
\]
\end{theorem}

\begin{remark} For $K=1$, algorithm \textsf{BIT} is entirely different than the Cover's algorithm \cite{cover1966behavior} but with the same regret guarantee.
\end{remark}

\begin{proof}
Step 1: 
For each $t$,
\[
\ell_t(p) = \max_{k=1,\dots,K} |p - f_t^{k}|,\qquad p\in[0,1].
\]
Hence \(\ell_t\) is convex and 1-Lipschitz on \([0,1]\), any subgradient \(s_t\in\partial\ell_t(p_t)\) satisfies \(|s_t|\le 1\).
Thus, the projected OGD algorithm as used in algorithm \textsf{BIT} with diameter \(D=1\) yields for any fixed \(p\in[0,1]\) satisfies  \cite{HazanBook}
\begin{equation}\label{eq:bin1}
\sum_{t=1}^T \ell_t(p_t) - \sum_{t=1}^T \ell_t(p)
\le \frac{D^2}{2\eta} + \frac{\eta}{2}\sum_{t=1}^T \|s_t\|^2
\le \frac{1}{2\eta} + \frac{\eta T}{2}.
\end{equation}

Choosing \(\eta = 1/\sqrt{T}\) gives
\begin{equation}\label{eq:bin2}
\sum_{t=1}^T \ell_t(p_t) \le \min_{p\in[0,1]}\sum_{t=1}^T \ell_t(p) + \sqrt{T}.
\end{equation}

Step 2:
Next, we connect the expected cost of \textsf{BIT} to the expectation of the surrogate cost $\sum_{t=1}^T \ell_t(p_t)$.


For each fixed \(k\) and fixed realization of the probability vector \(\bp=p_{1:T}\),
the conditional expectation equals
\[
\bbE\{S_k \mid \bp]
= \sum_{t=1}^T \bbE\{\mathbf{1}\{x_t\ne f_t^{(k)}\}\mid \bp]
= \sum_{t=1}^T |p_t - f_t^{(k)}|,
\]
since \(\Pr[x_t=1\mid \bp]=p_t\). 
Let
\(Z_k(\bp):=\bbE\{S_k\mid \bp\}=\sum_{t=1}^T |p_t-f_t^{(k)}|\). 
Then 
(i) Jensen's inequality implies that  

\begin{equation}\label{eq:bin3}
\max_k \bbE\{Z_k(\bp)\}
\le \bbE\left\{\max_k Z_k(\bp)\right\}.
\end{equation}

and
(ii) for each realization of \(\bp\), 
\begin{equation}\label{eq:bin4}
\max_k \sum_{t=1}^T |p_t-f_t^{(k)}|
\le \sum_{t=1}^T \max_k |p_t-f_t^{(k)}|
= \sum_{t=1}^T \ell_t(p_t).
\end{equation}



Thus, we have 
\begin{equation}\label{eq:bin5}
\max_k \bbE\{S_k\}
= \max_k \bbE\left\{\bbE\{S_k\mid p\}\right\}
= \max_k \bbE\{Z_k(p)\}
\stackrel{\eqref{eq:bin3}}{\le} \bbE\left\{\max_k Z_k(p)\right\}
\stackrel{\eqref{eq:bin4}}{\le} \bbE\left\{\sum_{t=1}^T \ell_t(p_t)\right\}.
\end{equation}


%Thus
%\[
%\boxed{\displaystyle \max_{k}\bbE\{S_k] \le \mathbb{E}\!\Big[\sum_{t=1}^T \ell_t(p_t)\right\}.}
%\]
%
%
%For each \(k\), let the cost be
%\[
%S_k = \sum_{t=1}^T \mathbf{1}\{x_t\ne f_t^{k}\}.
%\]
%Note that for each $t$, $\bbE\{ \mathbf{1}\{x_t\ne f_t^{k}\} \mid p_{1:T}\} = |p_t - f_t^{k}|$.
%Thus, linearity of expectation implies 
%\[
%\mathbb{E}\{S_k\mid p_{1:T}\} = \sum_{t=1}^T |p_t - f_t^{k}|.
%\]
%Since \(\ell_t(p_t)=\max_k |p_t - f_t^{k}|\),
%\[
%\max_{k}\mathbb{E}\{S_k\mid p_{1:T}\}
%\;=\; \max_k \sum_{t=1}^T |p_t - f_t^{k}|
%\;\le\; \sum_{t=1}^T \ell_t(p_t).
%\tag{3}
%\]
%Using the tower property, we moreover get 
%\[
%\max_{k}\mathbb{E}\{S_k\} \le \bbE\left\{ \sum_{t=1}^T \ell_t(p_t)\right\}.
%\tag{31}
%\]
We want an upper bound on \(\mathbb{E}\{\max_k S_k\}\), the expected cost of \textsf{BIT}. Towards that end, use the decomposition
\[
\max_k S_k
\le \max_k \mathbb{E}\{S_k\} + \max_k |S_k - \mathbb{E}\{S_k\}|.
\]
Taking expectations and using \eqref{eq:bin5} gives
\begin{equation}\label{eq:bin5a}
\bbE\{\max_k S_k]
\le \bbE\left\{\sum_{t=1}^T \ell_t(p_t)\right\} + \mathbb{E}\left\{\max_k |S_k - \mathbb{E}\{S_k\}|\right\}.
\end{equation}


We now bound the fluctuation term $\mathbb{E}\left\{\max_k |S_k - \mathbb{E}\{S_k\}|\right\}$. Note that for any vector \(a=(a_1,\dots,a_K)\),
\[
\max_k |a_k| \le \sqrt{\sum_{k=1}^K a_k^2}.
\]
Using this for \(a_k = S_k - \mathbb{E}\{S_k\}\) and taking expectations, we get
\begin{equation}\label{eq:bin6}
\mathbb{E}\left\{\max_k |S_k - \mathbb{E}\{S_k\}|\right\}
\le \mathbb{E}\left\{\sqrt{\sum_{k=1}^K (S_k-\mathbb{E}\{S_k\})^2}\right\}
\le \sqrt{\mathbb{E}\left\{\sum_{k=1}^K (S_k-\mathbb{E}\{S_k\})^2\right\}}
\end{equation}
where the last step uses Jensen's inequality.

Conditioned on the probability sequence $\bp$, the random variables
$\mathbf{1}\{x_t\ne s_t^{(k)}\}$ are independent Bernoulli random variables
with success probabilities
\[
q_t := \Pr[x_t\ne s_t^{(k)}\mid p_t] = |p_t - s_t^{(k)}|.
\]
Hence,
\[
\mathrm{Var}(S_k\mid p_{1:T})
= \sum_{t=1}^T \mathrm{Var}\big(\mathbf{1}\{x_t\ne s_t^{(k)}\}\mid p_t\big)
= \sum_{t=1}^T q_t(1-q_t).
\]
Since $q(1-q)\le \tfrac{1}{4}$ for all $q\in[0,1]$, it follows that
\[
\mathrm{Var}(S_k\mid \bp) \le \tfrac{T}{4}.
\]

Thus,  
\[
\mathbb{E}\left\{\sum_{k=1}^K (S_k-\mathbb{E}\{S_k\})^2\right\} \le \frac{K T}{4}.
\]
Therefore, from \eqref{eq:bin6},
\begin{equation}\label{eq:bin7}
\bbE\left\{\max_k |S_k - \mathbb{E}\{S_k\}|\right\} \le \sqrt{\frac{K T}{4}} = \frac{\sqrt{K T}}{2}.
\end{equation}


Plugging \eqref{eq:bin7} into \eqref{eq:bin5a} we obtain
\begin{equation}\label{eq:bin8}
\bbE\{C_{\textsf{BIT}}(T)\} = \bbE\{\max_k S_k] \le \bbE\left\{\sum_{t=1}^T \ell_t(p_t)\right\} + \frac{\sqrt{K T}}{2}.
\end{equation}



Step 3:
Finally, we connect the cost of $\opt$ to  $\min_{p\in[0,1]}\sum_{t=1}^T \ell_t(p)$  as follows.
For any fixed binary action \(x\in\{0,1\}\) and any round \(t\),
\[
\ell_t(x)=\max_{k}|x-f_t^{(k)}|
=\max_k \mathbf{1}\{x\ne f_t^{(k)}\}
=\mathbf{1}\{\exists k:\;x\ne f_t^{(k)}\}.
\]
Summing over \(t\) yields
\[
\sum_{t=1}^T \ell_t(x)
= \sum_{t=1}^T \mathbf{1}\{\exists k:\;x\ne f_t^{(k)}\}
\;\ge\; \max_{k}\sum_{t=1}^T \mathbf{1}\{x\ne f_t^{(k)}\},
\]
because picking the best index \(k\) for the sum can only decrease the total.
Therefore, since \(\{0,1\}\subset[0,1]\),
\begin{equation}\label{eq:bin9}
\min_{p\in[0,1]}\sum_{t=1}^T \ell_t(p)
\le \min_{b\in\{0,1\}}\sum_{t=1}^T \ell_t(b)
\le \min_{b\in\{0,1\}}\max_{k}\sum_{t=1}^T \mathbf{1}\{b\ne f_t^{(k)}\}
= C_\opt,
\end{equation}
as claimed.




Taking expectations in \eqref{eq:bin2} and using \eqref{eq:bin8} and \eqref{eq:bin9},
\[\bbE\{C_{\textsf{BIT}}\}  = \mathbb{E}\left\{\max_k S_k\right\}
\le \min_{p\in[0,1]}\sum_{t=1}^T \ell_t(p) + \sqrt{T} + \frac{\sqrt{K T}}{2}
\le C_\opt + \Big(1+\tfrac{\sqrt{K}}{2}\Big)\sqrt{T},
\]
which implies that 
$$R_{\textsf{BIT}}(T) \le O(\sqrt{KT})$$
proving the theorem.
\end{proof}

Note that the connection made in Step 2 between cost \textsf{BIT} and surrogate cost $\ell_t$ is also the intuition for considering an OGD algorithm with surrogate function $\ell_t$.

%\paragraph{High-probability remark.}
%The expectation bound above can be converted into a high-probability bound by applying Bernstein (or Hoeffding/Azuma) concentration to the deviations \(S_k-\mathbb{E}S_k\). Concretely, with probability at least \(1-\delta\),
%\[
%\mathrm{AlgCost}_K \le \min_{p\in[0,1]}\sum_{t=1}^T \ell_t(p) + \sqrt{T} + O\!\left(\sqrt{T\ln\frac{K}{\delta}}\right),
%\]
%and therefore
%\[
%\mathrm{AlgCost}_K \le \mathrm{OPT}_K + O\!\left(\sqrt{T\ln\frac{K}{\delta}} + \sqrt{T}\right).
%\]

%\begin{remark}[Why the probabilistic trick fails for convex losses]
%The probabilistic relaxation in Algorithm~\ref{alg:prob-ogd-K} crucially relies on the fact that,
%for binary outcomes, the expected $0$--$1$ loss is an \emph{affine} function of the mixing
%probability $p$, i.e.
%$\mathbb{E}_{x\sim\mathrm{Bern}(p)}[\mathbf{1}\{x\ne s_t\}]=|p-s_t|$.
%Consequently, the per-round surrogate
%$\ell_t(p)=\max_k|p-f_t^{k}|$ is convex and exactly matches the
%expected discrete loss, allowing OGD to operate on a one-dimensional convex function whose
%expectation equals the true loss.
%
%When $f_t$ and $g_t$ are general convex functions over a convex domain
%$\mathcal X\subset\mathbb R^d$, this correspondence breaks:
%if one samples $X_t\sim\mu_t$ and defines the analogue
%$\ell_t(\mu)=\max\{\mathbb{E}_{X\sim\mu}\{f_t(X)\},\,\mathbb{E}_{X\sim\mu}\{g_t(X)\}\}$,
%then
%\[
%\max\{\bbE\{f_t(X)\},\bbE\{g_t(X)\}\}
%\;\neq\;
%\bbE\{\max\{f_t(X),g_t(X)\}\},
%\]
%and convexity implies
%$f_t(\bbE\{X\})\le\bbE\{f_t(X)\}$,
%so randomization can only \emph{increase} the expected loss.
%Thus the binary proof technique no longer yields a valid surrogate whose expectation matches
%the discrete objective or whose comparator coincides with the deterministic benchmark
%$$\min_{x\in\mathcal X}\max\left\{\sum_t f_t(x),\sum_t g_t(x)\right\}.$$
%\end{remark}

%\begin{remark}[Tie-breaking can induce linear regret for FTL]
%\label{rem:tie-breaking}
%With two sequences $(f_t,g_t)$,  
%the FTL update becomes
%\[
%x_{t+1}=\arg\min_{x\in\{0,1\}}
%\max\Big\{\sum_{\tau=1}^t \mathbf{1}\{x\ne f_\tau\},\;
%          \sum_{\tau=1}^t \mathbf{1}\{x\ne g_\tau\}\Big\}.
%\]
%
%On the alternating adversarial input
%\((f_t,g_t)=(0,1),(1,0),(0,1),(1,0),\ldots\) the empirical objectives
%for the two constant actions are equal at every time \(t\):
%\[
%\max\Big\{\sum_{\tau=1}^t \1\{0\ne f_\tau\},\;\sum_{\tau=1}^t \1\{0\ne g_\tau\}\Big\}
%=
%\max\Big\{\sum_{\tau=1}^t \1\{1\ne f_\tau\},\;\sum_{\tau=1}^t \1\{1\ne g_\tau\}\Big\}.
%\]
%Hence FTL is indifferent at every step and its behavior is determined solely
%by the tie-breaking rule. If ties are broken by \emph{flipping} the previous
%action (or more generally so that \(x_t=t\bmod 2\)), then FTL chooses
%\(x_t=f_t\) for all \(t\) and thus
%\[
%C_{\mathrm{FTL}}(T)=\max\Big\{\sum_{t=1}^T\1\{x_t\ne f_t\},\;\sum_{t=1}^T\1\{x_t\ne g_t\}\Big\}=T,
%\]
%whereas the fixed-action benchmark satisfies \(C_\opt=T/2\). Therefore the regret of 
%FTL grows linearly in \(T\).
%\qedhere
%\end{remark}


\begin{remark}
When there is only one binary sequence $f_t$, drawn i.i.d.\ from a fixed
distribution,  FTL algorithm-which at each step
chooses the empirical majority of past $f_t$'s achieves $O(1)$ regret \cite{feder2002universal} since FTL's action stabilizes quickly over time on account of the law of large numbers.

In contrast, in presence of two sequences $(f_t,g_t)$ and cost \eqref{defn:costbit}, 
the FTL update becomes
\[
x_{t+1}=\arg\min_{x\in\{0,1\}}
\max\Big\{\sum_{\tau=1}^t \mathbf{1}\{x\ne f_\tau\},\;
          \sum_{\tau=1}^t \mathbf{1}\{x\ne g_\tau\}\Big\}.
\]
In the presence of two i.i.d. sequences, the FTL's action $x_{t+1}$ need not stabilize {\bf quickly enough}. To see this, consider the input 
where at each time \(t\),  \((f_t,g_t)\in\{0,1\}^2\) are generated i.i.d.\ according to distribution
\begin{equation}\label{eq:input-law-code}
\begin{aligned}
\Pr[(f_t,g_t) = (1,0)] &= \tfrac{1}{2} + \varepsilon - \delta,\\[4pt]
\Pr[(f_t,g_t) = (0,1)] &= \tfrac{1}{2} - \varepsilon - \delta,\\[4pt]
\Pr[(f_t,g_t) = (0,0)] &= \delta,\\[4pt]
\Pr[(f_t,g_t) = (1,1)] &= \delta,
\end{aligned}
\end{equation}
where
$\varepsilon = \frac{a}{\sqrt{T}}$, and $a, \delta$ are constants. For this input, with $a=2, \delta=0.02$, we plot the regret of FTL in Fig. \ref{fig:ftl-regret}, where its regret scales as $O(\sqrt{T})$. Compared to when there is a single binary sequence, with two sequences, the key difference  is that there are two competing empirical means, one for 
the sequence $\{f_t\}$ and another for $\{g_t\}$. 
Although each empirical mean concentrates around its expectation with fluctuations 
of order $O(1/\sqrt{t})$, their difference behaves like a one-dimensional random walk 
that crosses zero about $O(\sqrt{T})$ times. 
Each crossing causes the FTL algorithm to switch its decision, incurring a constant 
loss per switch. Consequently, the total regret grows as 
\[
R_{\textsf{FTL}}(T) = O(\sqrt{T}).
\]
\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=0.95]
\begin{axis}[
    width=8cm,
    height=6cm,
    xlabel={Time horizon $T$},
    ylabel={Mean regret $\mathbb{E}\{R_{\textsf{FTL}}(T)\}$},
    xmode=log,
    ymode=log,
    log basis x={10},
    log basis y={10},
    xtick={1e3,1e4,1e5,1e6},
    xticklabels={$10^3$,$10^4$,$10^5$,$10^6$},
    ytick={1,3,10,30,100,300},
    yticklabels={$1$,$3$,$10$,$30$,$100$,$300$},
    grid=both,
    grid style={gray!20},
    major grid style={gray!30},
    minor tick num=1,
    tick label style={font=\small},
    label style={font=\small},
    legend style={
        at={(0.03,0.97)},
        anchor=north west,
        draw=none,
        fill=none,
        font=\small
    },
]
% empirical mean regret
\addplot[
    mark=o,
    mark size=2.5pt,
    thick,
    color=blue
] coordinates {
    (1e3, 4.05)
    (1e4, 12.23)
    (1e5, 39.28)
    (1e6, 129.33)
};
\addlegendentry{Empirical mean regret}

% fitted sqrt(T) line: c * sqrt(T)
\addplot[
    dashed,
    color=red,
    thick
] coordinates {
    (1e3, {0.13*sqrt(1e3)})
    (1e6, {0.13*sqrt(1e6)})
};
\addlegendentry{$c\sqrt{T}$ fit, $c\!\approx\!0.13$}

\end{axis}
\end{tikzpicture}
\caption{Empirical growth of FTL’s regret on the i.i.d. mixture input with random tie-breaking.}
\label{fig:ftl-regret}
\end{figure}



%\begin{figure}[ht]
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%    width=9cm, height=6cm,
%    xlabel={Time horizon $T$},
%    ylabel={Regret},
%    xmode=log, ymode=log,
%    log basis x={10}, log basis y={10},
%    grid=both,
%    legend style={at={(0.97,0.03)},anchor=south east},
%    minor grid style={gray!20}, major grid style={gray!40}
%]
%% empirical data (example from simulation)
%\addplot+[ mark=*, mark size=2pt, blue]
%    coordinates {
%        (1000, 4.52)
%        (3000, 6.89)
%        (10000, 13.42)
%        (30000, 22.28)
%        (100000, 41.04)
%    };
%\addlegendentry{Empirical FTL regret ($\delta=0.1$)}
%
%% sqrt(T) trend
%%\addplot+[domain=1e3:1e5, samples=50, dashed, thick, red]
%   % {0.13*sqrt(x)};
%%\addlegendentry{$c\sqrt{T}$ reference}
%
%\end{axis}
%\end{tikzpicture}
%\caption{Empirical regret for FTL under i.i.d.\ inputs with small symmetric bias ($\varepsilon = a/\sqrt{T}$, $\delta=0.1$).}
%\label{fig:ftl-regret-delta}
%\end{figure}
%
%\begin{figure}[ht]
%\centering
%\begin{tikzpicture}[scale=1.0,>=stealth]
%
%% Axes for f_t
%\draw[->] (0,1.8) -- (10.5,1.8) node[below right] {$t$};
%\draw[->] (0,1.8) -- (0,3.2) node[left] {$f_t$};
%
%% Input sequence f_t (noisy binary pattern)
%\draw[thick,gray!70!black]
%  (0,2.0) -- (0.5,2.0) -- (0.5,3.0) -- (1.5,3.0) -- (1.5,2.0)
%  -- (2.0,2.0) -- (2.0,3.0) -- (3.5,3.0) -- (3.5,2.0)
%  -- (4.0,2.0) -- (4.0,3.0) -- (5.0,3.0) -- (5.0,2.0)
%  -- (6.0,2.0) -- (6.0,3.0) -- (8.0,3.0) -- (8.0,2.0)
%  -- (9.5,2.0) -- (9.5,3.0) -- (10,3.0);
%
%% Horizontal reference lines for f_t = 0,1
%\draw[dashed,gray!50] (0,2.0) -- (10,2.0);
%\draw[dashed,gray!50] (0,3.0) -- (10,3.0);
%
%\node[gray!60!black] at (-0.4,3.0) {\footnotesize 1};
%\node[gray!60!black] at (-0.4,2.0) {\footnotesize 0};
%\node[gray!60!black] at (-0.6,2.5) {\footnotesize $f_t$};
%
%% Axes for x_t (FTL actions)
%\draw[->] (0,0) -- (10.5,0) node[below right] {$t$};
%\draw[->] (0,0) -- (0,1.5) node[left] {$x_t$};
%
%% FTL decisions (oscillating step function)
%\draw[thick,blue]
%  (0,1) -- (1,1) -- (1,0) -- (2,0)
%  -- (2,1) -- (3,1) -- (3,0) -- (4,0)
%  -- (4,1) -- (5,1) -- (5,0) -- (6,0)
%  -- (6,1) -- (8,1) -- (8,0) -- (10,0);
%
%% Horizontal reference lines for x_t = 0,1
%\draw[dashed,gray!50] (0,1) -- (10,1);
%\draw[dashed,gray!50] (0,0) -- (10,0);
%
%\node[gray!60!black] at (-0.4,1.0) {\footnotesize 1};
%\node[gray!60!black] at (-0.4,0.0) {\footnotesize 0};
%\node[blue!70!black] at (-0.6,0.5) {\footnotesize $x_t$};
%
%% Red arrows marking FTL switches
%\foreach \x in {1,2,3,5,8}{
%  \draw[red,->,thick] (\x,0.5) -- ++(0,0.4);
%}
%
%% Annotations
%\node[blue!70!black] at (5,1.3) {\small FTL decisions oscillate};
%\node[gray!60!black] at (5,3.3) {\small Input $f_t$ fluctuates randomly};
%\node at (9.3,1.2) {\footnotesize stabilization};
%
%\end{tikzpicture}
%\caption{Illustration of FTL oscillations for small bias $\varepsilon = a/\sqrt{T}$.
%Noisy binary inputs $f_t$ cause frequent switching of $x_t$ before it stabilizes.}
%\end{figure}
%
\end{remark}

\section{IID across sequences}






==> CodeGlobalExpertsProblemK=_2,4,8,16,32,64_.tex <==
import numpy as np
import matplotlib.pyplot as plt

np.random.seed(42)


# ===== BENIGN LOSS MODEL =====
def generate_benign_losses(T, K, low=0.2, high=0.8):
    return np.random.uniform(low, high, size=(T, K))


# ===== OFFLINE OPTIMAL (Best Expert) =====
def offline_minimal(losses):
    total_losses = np.sum(losses, axis=0)
    best_expert = np.argmin(total_losses)
    return best_expert, total_losses[best_expert]


# ===== BASE CASE MULTI K=2 =====
def multi_base(losses):
    T = losses.shape[0]
    p = np.ones(2) / 2
    p_hist = np.zeros((T, 2))
    for t in range(T):
        p_hist[t] = p.copy()
        diff = losses[t, 1] - losses[t, 0]
        p[0] += (p[1] * diff) / np.sqrt(T)
        p[1] += (p[0] * -diff) / np.sqrt(T)
        p = np.clip(p, 0, 1)
        p /= np.sum(p)
    return p_hist


# ===== MULTI for any K = 2^n =====
def multi_recursive(losses):
    T, K = losses.shape
    assert (K & (K - 1) == 0) and K > 0, "K must be a power of 2"

    if K == 2:
        return multi_base(losses)

    mid = K // 2
    p_left = multi_recursive(losses[:, :mid])
    p_right = multi_recursive(losses[:, mid:])
    p_comb = multi_base(np.column_stack([p_left[:, 0], p_right[:, 0]]))

    p_hist = np.zeros((T, K))
    for t in range(T):
        for i in range(mid):
            p_hist[t, i] = p_comb[t, 0] * p_left[t, i]
        for i in range(mid, K):
            p_hist[t, i] = p_comb[t, 1] * p_right[t, i - mid]
    return p_hist


# ===== ALGORITHM A =====
def algorithm_A_general(losses, eta_H=None, eta_O=None):
    T, K = losses.shape
    alpha = np.ones(K) / K
    p_hist = np.zeros((T, K))
    theta = 0.5

    if eta_H is None:
        eta_H = lambda t: 1.0 / np.sqrt(t + 1)
    if eta_O is None:
        eta_O = lambda t: 1.0 / np.sqrt(t + 1)

    for t in range(T):
        p_hist[t] = alpha.copy()
        grad_theta = losses[t, 0] - losses[t, 1]
        theta -= eta_O(t) * grad_theta
        theta = np.clip(theta, 0, 1)
        alpha[0] = theta
        alpha[1] = 1 - theta
        if K > 2:
            alpha[2:] = (1 - theta) / (K - 2)
        alpha /= np.sum(alpha)
    return p_hist, theta


# ===== RUN EXPERIMENT FOR MULTIPLE K and T =====
def run_experiment_K_T(K_values, T_values, runs=50):
    results = {}
    for K in K_values:
        print(f"\n=== Running for K={K} ===")
        multi_regrets = []
        a_regrets = []
        for T in T_values:
            multi_run = []
            a_run = []
            offline_run = []
            for _ in range(runs):
                losses = generate_benign_losses(T, K)
                best_expert, Lstar = offline_minimal(losses)
                offline_run.append(Lstar)

                p_multi = multi_recursive(losses)
                p_A, _ = algorithm_A_general(losses)

                loss_multi = np.sum(np.sum(p_multi * losses, axis=1))
                loss_A = np.sum(np.sum(p_A * losses, axis=1))

                regret_multi = loss_multi - Lstar
                regret_A = loss_A - Lstar

                multi_run.append(regret_multi)
                a_run.append(regret_A)

            multi_regrets.append(np.mean(multi_run))
            a_regrets.append(np.mean(a_run))
            print(f"T={T} | MULTI Regret={np.mean(multi_run):.4f} | Algorithm A Regret={np.mean(a_run):.4f} | Offline Opt Cost={np.mean(offline_run):.4f}")

        results[K] = {
            "T_values": T_values,
            "MULTI": multi_regrets,
            "AlgorithmA": a_regrets
        }

    return results


# ===== PLOT RESULTS =====
def plot_results(results, T_values):
    plt.figure(figsize=(10, 6))
    for K, data in results.items():
        plt.plot(T_values, data["MULTI"], marker='o', label=f"MULTI K={K}")
        plt.plot(T_values, data["AlgorithmA"], marker='x', linestyle='--', label=f"Algorithm A K={K}")
    plt.xlabel("T")
    plt.ylabel("Average Regret")
    plt.title("Regret Comparison for MULTI and Algorithm A")
    plt.legend()
    plt.grid(True)
    plt.show()


# ===== MAIN =====
if __name__ == "__main__":
    K_values = [2, 4, 16, 32, 64]
    T_values = [1000, 2000, 4000, 8000]
    results = run_experiment_K_T(K_values, T_values, runs=50)
    plot_results(results, T_values)

==> GlobalExperts.tex <==
\section{Improved result on GlobalExpertsProblem with i.i.d. input \cite{MannorGlobal}}
Let $\cX = \Delta_K$, the $K$-dimensional simplex, and writing $f_t^k(x) = x_k \ell_k(t)$, where $x_k$ is the $k$-th coordinate of $x\in \cX$, $\ell_k(t)$ is the loss corresponding to the $k$-th expert, and $k=1,2\dots, K$, we get the GlobalExpertsProblem \cite{MannorGlobal} with $K$ experts in the i.i.d. input case  is a  special case of our problem \eqref{defn:expregretintro}.
Thus, from Remark \ref{rem:multipleK}, we get that the expected {\it min-max} static regret of Algorithm \ref{alg:main} is $O(\sqrt{T\log K})$ for the GlobalExpertsProblem with i.i.d. input. In comparison, \cite{MannorGlobal} 
derived a {\it min-max} static regret \eqref{intro-moregret-def} guarantee of 
$O(\sqrt{T}\log K)$ with adversarial input for the following algorithm called {\textsf MULTI}: 
For $K=2$, $$x_1(t+1) = x_1(t) + \frac{x_2(t) \ell_2(t) - x_1(t) \ell_1(t)}{\sqrt{T}},$$ and $x_2(t) = 1-x_1(t)$. 
For general $K$, the $K=2$ algorithm was used recursively.
%More than the slightly improved guarantee in the i.i.d. input, the main advantage of our approach is the simplicity and elegance of the proof, which is rather involved in \cite{MannorGlobal}. 
Compared to our Algorithm \ref{alg:main}, the {\textsf MULTI} algorithm \cite{MannorGlobal} is  very compute intensive  since it recursively uses an algorithm for $K=2$ and requires the knowledge of time horizon $T$.

==> K-ExpertsHedgeCodeFunctionofK.tex <==
import numpy as np
import matplotlib.pyplot as plt

class Hedge:
    def __init__(self, K, eta):
        self.K = K
        self.eta = eta
        self.weights = np.ones(K)

    def predict(self):
        return self.weights / np.sum(self.weights)

    def update(self, losses):
        self.weights *= np.exp(-self.eta * losses)
        self.weights /= np.sum(self.weights)  # normalization for stability

def simulate_hedge(K=10, T=200, eta=0.5):
    hedge = Hedge(K, eta)
    regrets = []
    cumulative_loss_alg = 0

    np.random.seed()  # new seed for each run
    losses_matrix = np.random.rand(K, T)

    cumulative_losses_experts = np.zeros(K)

    for t in range(T):
        probs = hedge.predict()
        losses = losses_matrix[:, t]

        loss_alg = np.dot(probs, losses)
        cumulative_loss_alg += loss_alg

        cumulative_losses_experts += losses
        best_loss = np.min(cumulative_losses_experts)

        regrets.append(cumulative_loss_alg - best_loss)
        hedge.update(losses)

    return regrets

def simulate_multiple_runs(K, T, eta, runs=50):
    all_regrets = []
    for run in range(runs):
        regrets = simulate_hedge(K, T, eta)
        all_regrets.append(regrets)

    avg_regret = np.mean(all_regrets, axis=0)
    return avg_regret

if __name__ == "__main__":
    Ks = [10, 100, 1000, 10000]
    T = 200
    eta = 0.5
    runs = 50

    plt.figure(figsize=(10, 6))

    for K in Ks:
        print(f"Running Hedge simulation for K={K} with {runs} runs...")
        avg_regrets = simulate_multiple_runs(K, T, eta, runs=runs)
        plt.plot(avg_regrets, label=f"K={K}")

    plt.xlabel("Time step")
    plt.ylabel("Average Regret")
    plt.title(f"Hedge Algorithm Regret Over Time ({runs} runs per K)")
    plt.legend()
    plt.grid(True)
    plt.show()

==> LinearRegretOGDHedge.tex <==

\section{Linear Regret for OGD+{\it Hedge} in the adversarial input model }\label{app:lbogd+hedge}
Similar to the regret decomposition \eqref{defn:regretdecomp}, removing expectations, we can write the {\it min-max} static regret \eqref{intro-moregret-def} in the adversarial case as  
\begin{equation}\label{eq:regret_decomp}
R_T(\mathcal{A}) =
R_1 + R_2 + R_3,
\end{equation}
where
\[
R_1 = \max_{\theta\in \Delta_2} \sum_{t=1}^T \Lambda_t(x_t,\theta) - \sum_{t=1}^T \Lambda_t(x_t,\theta_t),
\]
is the regret corresponding to OGD for fixed $\theta_t$
\[
R_2 = \sum_{t=1}^T \Lambda_t(x_t,\theta_t) - \min_{x\in \mathcal{X}} \sum_{t=1}^T \Lambda_t(x,\theta_t),
\]
is the regret corresponding to {\it Hedge} for losses coming from $\lambda_t=(f_t, g_t)$, and 
\[
R_3 = \min_{x\in \mathcal{X}} \sum_{t=1}^T \Lambda_t(x,\theta_t) - C_\opt.
\]
With the use of OGD and {\it Hedge} algorithms, both  $R_1 = O(\sqrt{T})$, $R_2 = O(\sqrt{T})$ following standard OGD and {\it Hedge} guarantees \cite{HazanBook}, 
however, the problem term is $R_3$.
To illustrate that, corresponding to the chosen input, 
\[
f_{2j}(x) = L - L x, \quad f_{2j+1}(x) = x, \quad 
g_{2j}(x) = x, \quad g_{2j+1}(x) = L + L x, \quad j=0,\dots,T/2-1.
\]
we define the per-pair duality gap
\[
\delta_j := \min_{x\in\mathcal{X}} \big( \Lambda_{2j}(x,\theta_{2j}) + \Lambda_{2j+1}(x,\theta_{2j+1}) \big)
- \min_{x\in\mathcal{X}} \max_{\theta\in\Delta_2} \big( \Lambda_{2j}(x,\theta) + \Lambda_{2j+1}(x,\theta) \big).
\]

such that 
\[
R_3 = \sum_{j=0}^{T/2-1} \delta_j.
\]

With the chosen input, the optimal dual weight\footnote{It is non-unique.} is $\theta^\star = (0.5,0.5)$ and $x^\star=0$, and the mismatch  between the algorithm’s adaptation speed and the input’s alternating slopes
results in  
$\delta_j \approx O(1)$ for $O(T)$ time slots
inducing linear growth of $R_3$ with respect to $T$ and consequently resulting in linear regret for OGD+{\it Hedge} as exhibited in Figure \ref{fig:linearregret}. 


==> LowerBoundOGD+Hedge.tex <==
%\documentclass[12pt]{article}
%\usepackage{amsmath, amssymb, amsfonts, geometry}
%\geometry{margin=1in}
%\input{input}
%\begin{document}
%
%\section*{Linear Regret of OGD + Hedge under Alternating Linear Losses}
%
%\subsection*{Setup}
%
%Let $T = 2N$ and $\mathcal{X} = [0,1]$. Define the convex linear losses:
%\[
%\begin{aligned}
%f_{2j-1}(x) &= 1.2 - 0.2 x, & f_{2j}(x) &= x, \\
%g_{2j-1}(x) &= x, & g_{2j}(x) &= 0.8 + 0.2 x,
%\end{aligned}
%\quad j=1,\dots,N.
%\]
%
%The learner selects $x_t \in [0,1]$ using OGD, while Hedge maintains a weight vector $\theta_t \in \Delta_2$.  
%The total cost of the algorithm is
%\[
%\mathrm{ALG} = \sum_{t=1}^T \max\{f_t(x_t), g_t(x_t)\},
%\]
%and the offline benchmark is
%\[
%\mathrm{OPT} = \min_{x\in[0,1]} \max\Big\{\sum_{t=1}^T f_t(x), \sum_{t=1}^T g_t(x)\Big\}.
%\]
%
%\subsection*{Step 1: Offline optimum}
%
%For each pair $(2j-1,2j)$,
%\[
%\begin{aligned}
%f_{2j-1}(x)+f_{2j}(x) &= 1.2 - 0.2x + x = 1.2 + 0.8x,\\
%g_{2j-1}(x)+g_{2j}(x) &= x + 0.8 + 0.2x = 0.8 + 1.2x.
%\end{aligned}
%\]
%
%Thus,
%\[
%\sum_{t=1}^T f_t(x) = N(1.2 + 0.8x), \quad
%\sum_{t=1}^T g_t(x) = N(0.8 + 1.2x).
%\]
%
%The benchmark is
%\[
%\mathrm{OPT} = \min_{x\in[0,1]} \max\{N(1.2 + 0.8 x), N(0.8 + 1.2 x)\}.
%\]
%
%Since both functions are increasing in $x$, the minimum occurs at $x=0$, giving
%\[
%\mathrm{OPT} = N \cdot 1.2.
%\]
%
%\subsection*{Step 2: Loss gaps per round}
%
%Define the optimal point for each round:
%\[
%x^\star_{2j-1} = 0 \quad (\text{minimizes } f_{2j-1}), \qquad
%x^\star_{2j} = 1 \quad (\text{minimizes } g_{2j}).
%\]
%
%The difference between the losses for odd rounds:
%\[
%f_{2j-1}(x) - g_{2j-1}(x) = 1.2 - 1.2 x \ge 0, \quad x \in [0,1],
%\]
%so $f$ is the “better expert”.
%
%For even rounds:
%\[
%g_{2j}(x) - f_{2j}(x) = 0.8 - 0.8 x \ge 0,
%\]
%so $g$ is the “better expert”.
%
%\subsection*{Step 3: Effect of step sizes $\eta_x, \eta_\theta = 1/\sqrt{T}$}
%
%- OGD step size: $|x_{t+1} - x_t| \le \eta_x \|\nabla \ell_t\| = O(1/\sqrt{T})$.
%- Hedge update: $|\theta_{t+1} - \theta_t| = O(\eta_\theta) = O(1/\sqrt{T})$.
%
%Even with these small updates, the **optimal expert alternates every round**. Hence the algorithm cannot track the min–max optimum:
%
%\[
%|x_t - x^\star_t| \ge |x^\star_{2j} - x^\star_{2j-1}| - O(T \cdot 1/\sqrt{T}) = 1 - O(1/\sqrt{T}) \approx \Theta(1).
%\]
%
%Similarly, Hedge weights remain near uniform $\theta_t \approx (1/2,1/2)$.
%
%\subsection*{Step 4: One-round regret lower bound}
%
%Let $e_t^\star$ be the “best expert” at round $t$. Then
%\[
%\max\{f_t(x_t), g_t(x_t)\} - \min\{f_t(x^\star), g_t(x^\star)\} 
%\ge |f_t(x_t) - f_t(x^\star_t)| \quad \text{or} \quad |g_t(x_t) - g_t(x^\star_t)|.
%\]
%
%Since $|x_t - x^\star_t| = \Theta(1)$ and $|\nabla f_t|, |\nabla g_t| = \Theta(1)$,
%\[
%\text{one-round regret} = \Omega(1).
%\]
%
%\subsection*{Step 5: Cumulative regret}
%
%Summing over $T$ rounds:
%\[
%\mathrm{Regret} = \sum_{t=1}^T \Big(\max\{f_t(x_t), g_t(x_t)\} - \text{OPT}/T\Big) = \Omega(T).
%\]
%
%\subsection*{Conclusion}
%
%Even if we set $\eta_x, \eta_\theta = 1/\sqrt{T}$, the algorithm **cannot track the alternating optimum**, and the cumulative regret scales linearly:
%
%\[
%\boxed{\mathrm{Regret} = \mathrm{ALG} - \mathrm{OPT} = \Omega(T)}.
%\]
%
%\newpage
\subsection{Lower Bound on {\it min-max} static regret for OGD+{\it Hedge}}
In this subsection, we show that OGD+{\it Hedge}\footnote{See Section \ref{sec:hedgeintro} for basic definition of the Experts Problem and the {\it Hedge} algorithm).} that is a natural algorithm to solve \eqref{intro-moregret-def} suffers linear regret.
Recall the definition of $C_\opt = \min_x \max_\theta \sum_{t=1}^T \Lambda_t(x,\theta)$ from \eqref{defn:optcostintro}, where $\Lambda_t(x,\theta) = \theta_1 f_t + \theta_2g_t$.
Thus, to find the optimal pair $(x^\star, \theta^\star)$ that optimizes $C_\opt$, a natural algorithm is to use OGD with objective function $\theta_{t1} f_t(x) + \theta_{t2}g_t(x)$ with step size $\eta_x$ to find the action $x_t$ and use  
{\it Hedge} to update weights $(\theta_{t1}, \theta_{t2}) \in \Delta_2$ with losses $f_t, g_t$ and step size $\eta_\theta$. 

We next show that OGD+{\it Hedge} suffers linear {\it min-max} static regret \eqref{intro-moregret-def}.
Towards that end, we consider the input defined as follows. Let $\cX = [0,1]$ and define $T/2$ pairs of rounds $(2j,2j+1)$ with the following losses:
\[
f_{2j}(x) = L - L x, \quad f_{2j+1}(x) = x, \quad 
g_{2j}(x) = x, \quad g_{2j+1}(x) = L + L x, \quad j=0,\dots,T/2-1.
\] 
The guiding principle behind this input is:
\begin{enumerate}
    \item \textbf{Alternating conflicting objectives:} Each consecutive pair of rounds is designed so that minimizing $f_t$ and $g_t$ requires opposite actions, forcing the algorithm to constantly trade off between the two losses.
    \item \textbf{Linear separation:} The functions are linear with slopes of opposite signs, ensuring that the offline optimum can pick a fixed $x^\star$ to balance the sums, while any online algorithm that acts causally incurs a constant per-round loss.
\end{enumerate}

For this input with $L=10$, we calculate the regret of OGD+{\it Hedge}  in Table~\ref{tab:regret} with step sizes 
$\eta_x = \eta_\theta = 1/\sqrt{T}$ and visualize it in Figure~\ref{fig:linearregret}, that clearly shows that the {\it min-max} static regret scales linearly with $T$. The conceptual reasons for this linear regret scaling are detailed in Appendix \ref{app:lbogd+hedge}. 

\begin{remark}
Similarly, one can construct an input example for which the other appealing algorithm, {\bf primal-dual} that does primal-descent in $x$ space and primal ascent in $\theta$ space with function $\Lambda_t(x,\theta)$ also suffers a linear regret. We acknowledge that this is not a complete characterization for all online algorithms, 
but  proving a $\Omega(T)$ lower bound with non-adaptive input that is applicable for all online algorithms is too challenging.
\end{remark}
%\begin{table}[h]
%\centering
%\begin{tabular}{c|c}
%\hline
%$T$ & Final Cumulative Regret $R_T$ \\
%\hline
%200   & 1055.27 \\
%400   & 2118.70 \\
%800   & 4258.55 \\
%1600  & 8555.98 \\
%3200  & 17181.09 \\
%\hline
%\end{tabular}
%\caption{Final cumulative regret of OGD+Hedge on strongly adversarial input.}
%\label{tab:regret}
%\end{table}
%
%\begin{figure}[h!]
%\centering
%\begin{tikzpicture}
%\begin{axis}[
%    xlabel={Round $t$},
%    ylabel={Cumulative Min-Max Regret},
%    legend pos=north west,
%    grid=major,
%    width=12cm,
%    height=7cm
%]
%\addplot coordinates {(200,1055.27) (400,2118.70) (800,4258.55) (1600,8555.98) (3200,17181.09)};
%\addlegendentry{$R_T$ vs $T$}
%\end{axis}
%\end{tikzpicture}
%\caption{Cumulative regret grows roughly linearly with $T$, confirming $R_3 = \Omega(T)$.}
%\label{fig:linearregret}
%\end{figure}
\begin{table}[h!]
\centering
\begin{tabular}{c|c}
\hline
$T$ & Cumulative Regret $R_T$ \\
\hline
100       & 133.3 \\
1,000     & 949.0 \\
10,000    & 9530.4 \\
100,000   & 95431.1 \\
1,000,000 & 954310.0 \\
\hline
\end{tabular}
\caption{Cumulative regret of OGD+Hedge on the linear lower-bound input with $L=10$ and step sizes $\eta_x=\eta_\theta=1/\sqrt{T}$. The regret grows roughly linearly with $T$.}
\label{tab:regret}
\end{table}

%\begin{figure}[h!]
%\centering
%\begin{tikzpicture}
%\begin{loglogaxis}[
%    xlabel={$T$},
%    ylabel={Cumulative Regret $R_T$},
%    grid=both,
%    width=0.8\textwidth,
%    height=0.5\textwidth,
%    legend pos=north west
%]
%\addplot[
%    color=blue,
%    mark=o,
%    thick
%] coordinates {
%    (100, 209.41)
%    (1000, 2551.54)
%    (10000, 26854.75)
%    (100000, 272641.03)
%    (1000000, 2739276.95)
%};
%\addlegendentry{OGD+Hedge, $L=10$}
%\end{loglogaxis}
%\end{tikzpicture}
%\caption{Cumulative regret of OGD+Hedge on the linear lower-bound input in log-log scale. The slope $\approx 1$ confirms that the regret grows linearly with $T$.}
%\label{fig:linearregret}
%\end{figure}

\begin{figure}
\begin{tikzpicture}
\begin{axis}[
title={expected {\it min-max} static  regret for OGD+Hedge (L=10.0)},
xlabel={Time Horizon T (log scale)},
ylabel={Regret 
  (log scale)},
xmode=log,
ymode=log,
legend pos=north west,
grid=both,
minor grid style={gray!25},
major grid style={gray!50},
width=10cm,
height=7cm,
]

% Data for OGD+Hedge Simulation Regret (R_T)
\addplot[
color=blue,
mark=*,
line width=1pt
]
table[row sep=\space, y index=1] {
T R_T
100 133.3
1000 949.0
10000 9530.4
100000 95431.1
1000000 954310.0
};
\addlegendentry{OGD+Hedge Simulation}

% Theoretical O(sqrt(T)) Scaled (R_T = 10 * sqrt(T))
\addplot[
color=red,
dashed,
line width=1pt
]
table[row sep=\space, y index=1] {
T R_T_theory
100 100.0
1000 316.2
10000 1000.0
100000 3162.3
1000000 10000.0
};
\addlegendentry{Theoretical $O(\sqrt{T}
 )$ Scaled}
\end{axis}
\end{tikzpicture}

\caption{Expected {\it min-max} regret of OGD+Hedge on the linear lower-bound input in log-log scale. The slope $\approx 1$ confirms that the regret grows linearly with $T$, starting point $x_0=0.5$ and $\theta = (0.5, 0.5)$.}
\label{fig:linearregret}
\end{figure}


%To exhibit this concretely, we next present the exact regret performance of OGD+{\it Hedge}  on this input 

\begin{comment}
\begin{theorem}\label{thm:univlb}
The {\it min-max} static regret of any online algorithm is $\Omega(T)$.
\end{theorem}
\begin{proof} 
To show the result, we modify the input \eqref{eq:lb1} as follows.
Consider the decision set $\cX = [0,1]$ and horizon $T = 2N$.
Define two possible environments, $A$ and $B$, each chosen with probability $1/2$ at the start by the adversary.

\paragraph{Environment A:}
For each $j = 1,\dots,N$,
\[
\begin{cases}
f_{2j-1}(x) = 1.2 - 0.2x, & f_{2j}(x) = x, \\[4pt]
g_{2j-1}(x) = x, & g_{2j}(x) = 0.8 + 0.2x.
\end{cases}
\]

\paragraph{Environment B:}
Each function is obtained by reflecting $x \mapsto 1-x$ in Environment~A:
\[
\begin{cases}
f_{2j-1}(x) = 1.0 + 0.2x, & f_{2j}(x) = 1 - x, \\[4pt]
g_{2j-1}(x) = 1 - x, & g_{2j}(x) = 0.2 + 0.2x.
\end{cases}
\]

Let $\cA$ be any (possibly randomized) online algorithm that selects $x_t \in [0,1]$.  
Its cost under environment $E \in \{A,B\}$ is
\[
C_{\cA}(E)
= 
\max\Biggl\{
\sum_{t=1}^T f_t^{E}(x_t),~
\sum_{t=1}^T g_t^{E}(x_t)
\Biggr\},
\]
and the static offline optimal cost is
\[
C_\opt(E)
=
\min_{x \in [0,1]}
\max\Biggl\{
\sum_{t=1}^T f_t^{E}(x),~
\sum_{t=1}^T g_t^{E}(x)
\Biggr\}.
\]

%Then, the expected regret of $\cA$ satisfies
%\[
%\mathbb{E}\left\{C_{\cA}(E) - C_\opt(E)\right\}
%~\ge~
%0.15T,
%\]
%i.e.\ the regret is $\Omega(T)$.
%\end{theorem}

\begin{proof}
Let $a_j = x_{2j-1}$ and $b_j = x_{2j}$ denote the algorithm's plays in pair $j$.
Define for Environment~A:
\[
\begin{aligned}
F_A(a,b) &= f^A_{2j-1}(a) + f^A_{2j}(b) = 1.2 - 0.2a + b,\\
G_A(a,b) &= g^A_{2j-1}(a) + g^A_{2j}(b) = a + 0.8 + 0.2b.
\end{aligned}
\]
Similarly, for Environment~B:
\[
\begin{aligned}
F_B(a,b) &= f^B_{2j-1}(a) + f^B_{2j}(b) = 2.0 + 0.2a - b,\\
G_B(a,b) &= g^B_{2j-1}(a) + g^B_{2j}(b) = 2.0 - a - 0.2b.
\end{aligned}
\]

The total costs in each environment are
\[
C_\cA(A) = \max\!\Bigl\{ S_F^A, S_G^A \Bigr\}, \qquad
C_\cA(B) = \max\!\Bigl\{ S_F^B, S_G^B \Bigr\},
\]
where $S_F^A = \sum_{j=1}^N F_A(a_j,b_j)$ and $S_G^A = \sum_{j=1}^N G_A(a_j,b_j)$
(and similarly for $B$).

The adversary chooses $A$ or $B$ {\bf uniformly at random} at the start,
so the algorithm’s expected cost is
\[
\mathbb{E}\left\{C_{\cA}(E)\right\} = \tfrac{1}{2}\bigl(C_\cA(A) + C_\cA(B)\bigr).
\]

Using the inequality $\max\{u,v\} \ge \tfrac12(u+v)$, we obtain
\[
\begin{aligned}
C_\cA(A) &\ge \tfrac12(S_F^A + S_G^A),\\
C_\cA(B) &\ge \tfrac12(S_F^B + S_G^B).
\end{aligned}
\]
Hence
\[
\mathbb{E}\left\{C_{\cA}(E)\right\}
~\ge~
\tfrac{1}{4}\bigl(S_F^A + S_G^A + S_F^B + S_G^B\bigr).
\]

Now, for any pair $(a,b)$,
\[
\begin{aligned}
F_A(a,b) + G_A(a,b) &= (1.2-0.2a+b) + (a+0.8+0.2b)
= 2.0 + 0.8a + 1.2b,\\[4pt]
F_B(a,b) + G_B(a,b) &= (2.0+0.2a-b) + (2.0 - a - 0.2b)
= 4.0 - 0.8a - 1.2b.
\end{aligned}
\]
Summing gives
\[
(F_A(a,b) + G_A(a,b)) + (F_B(a,b) + G_B(a,b)) = 6.0,
\]
independent of $a,b$.
Therefore,
\[
S_F^A + S_G^A + S_F^B + S_G^B = 6N,
\]
and hence
\[
\mathbb{E}\left\{C_{\cA}(E)\right\} \ge \frac{6N}{4} = 1.5N.
\]

Next, compute the offline optimal cost.
In both environments,
\[
C_\opt(E)
= \min_{x\in[0,1]}
\max\bigl\{
f_{2j-1}^{E}(x)+f_{2j}^{E}(x),
g_{2j-1}^{E}(x)+g_{2j}^{E}(x)
\bigr\}
= 1.2N.
\]
Thus
\[
\mathbb{E}\left\{C_{\cA}(E) - C_\opt(E)\right\} \ge (1.5 - 1.2)N = 0.3N = 0.15T,
\]
which implies that the {\it min-max} static regret for any online algorithm $\cA$ is $\Omega(T)$ when the input is chosen adversarially.
\end{proof}
\end{comment}
%\end{document}


==> Markov.tex <==
\section{Markovian Inputs}
\label{sec:markov}

In this section, we extend our main result (Theorem \ref{thm:main} of Section \ref{sec:iid})
to the setting where the loss sequence evolves according to a stationary Markov process.
Unlike the Martingale difference case, temporal dependence introduces an unavoidable bias
term that scales with the mixing time of the underlying Markov chain.

\subsection{Model}

Let $\{S_t\}_{t\ge 1}$ be a time-homogeneous, ergodic Markov chain on a measurable
state space $\cS$ with transition kernel $P$ and stationary distribution $\pi$.
We assume the chain is \emph{uniformly ergodic}, i.e., there exist constants
$C>0$ and $\tau_{\mathrm{mix}}>0$ such that for any initial distribution $\nu$,
\[
\|\nu P^t-\pi\|_{\mathrm{TV}} \le C e^{-t/\tau_{\mathrm{mix}}}, \qquad \forall t\ge 1.
\]

Let $\lambda:\cX\times\cS\to\mathbb R^2$ be a measurable mapping and define
\[
\lambda_t(x) := \lambda(x,S_t) = (f_t(x),g_t(x)).
\]
We assume that $f_t$ and $g_t$ satisfy Assumptions~\ref{cvx} and \ref{bddness}.

Define the stationary mean
\begin{equation}
\label{eq:markov_mu}
\mu(x)
:=
\mathbb E_{\pi}[\lambda(x,S)],
\qquad \forall x\in\cX,
\end{equation}
which is independent of $t$ by stationarity.

\subsection{Benchmarks}

Recall the benchmark
\begin{equation}
\label{eq:COPT_markov}
\bbE\{C_{\opt}\}
=
\bbE\!\left[
\min_{x\in \cX}
\max\!\left\{
\sum_{t=1}^T f_t(x),\;
\sum_{t=1}^T g_t(x)
\right\}
\right],
\end{equation}
and the deterministic surrogate benchmark
\begin{equation}
\label{eq:CbarOPT_markov}
\bar C_{\opt}
=
T \min_{x\in \cX} \max_{\theta\in\Delta_2} \theta^\top \mu(x).
\end{equation}

Unlike the i.i.d.\ case, $\bar C_{\opt}$ is \emph{not} equal to $\bbE\{C_{\opt}\}$ even
asymptotically; rather, it serves as a deterministic relaxation benchmark whose gap
depends on the mixing time.

\subsection{Gap between the benchmarks}

\begin{lemma}[Benchmark Gap under Markovian Inputs]
\label{lem:markov_benchmark_gap}
Under the Markovian model above and Assumptions~\ref{cvx} and \ref{bddness},
\[
\bigl|\bbE\{C_{\opt}\} - \bar C_{\opt}\bigr|
\;\le\;
O(\sqrt{T\log T}) + O(\tau_{\mathrm{mix}}).
\]
\end{lemma}

\begin{proof}
The proof follows Appendix~\ref{app:regretconnection} and
Lemma~\ref{lem:md_benchmark_gap}, with the sole modification that concentration of
$\sum_{t=1}^T \lambda_t(x)$ around $T\mu(x)$ now uses Markov-chain concentration
instead of independence.
Specifically, Lemma~\ref{lem:markov_concentration} shows that for any fixed $x\in\cX$,
\[
\mathbb E\!\left\{
\Big\|
\sum_{t=1}^T \lambda_t(x) - T\mu(x)
\Big\|_\infty
\right\}
=
O(\sqrt{T\log T}) + O(\tau_{\mathrm{mix}}).
\]
All minimax and $\varepsilon$--net arguments remain unchanged from
Appendix~\ref{app:regretconnection}, yielding the stated bound.
\end{proof}

\begin{lemma}[Concentration for additive functionals of Markov chains]
\label{lem:markov_concentration}
Let $\{S_t\}_{t\ge1}$ be a uniformly ergodic Markov chain with stationary distribution $\pi$
and mixing time $\tau_{\mathrm{mix}}$.
Assume $\|\lambda(x,S)\|_\infty\le B$ for all $(x,S)$.
Then for any fixed $x\in\cX$,
\[
\mathbb E\!\left[
\Big\|
\sum_{t=1}^T \lambda_t(x) - T\mu(x)
\Big\|_\infty
\right]
=
O(\sqrt{T\log T}) + O(\tau_{\mathrm{mix}}).
\]
\end{lemma}

\begin{proof}
Decompose
\[
\sum_{t=1}^T \lambda_t(x) - T\mu(x)
=
\sum_{t=1}^T \big(\lambda_t(x)-\mathbb E[\lambda_t(x)]\big)
+
\sum_{t=1}^T \big(\mathbb E[\lambda_t(x)]-\mu(x)\big).
\]

The second term is bounded using uniform ergodicity:
\[
\|\mathbb E[\lambda_t(x)]-\mu(x)\|_\infty
\le 2B\,\|\Law(S_t)-\pi\|_{\mathrm{TV}}
\le 2BC e^{-t/\tau_{\mathrm{mix}}},
\]
which yields an $O(\tau_{\mathrm{mix}})$ contribution after summation.

The first term is a centered additive functional of a uniformly ergodic Markov chain.
Expectation bounds follow by integrating standard tail inequalities
(e.g., \cite{paulin2015concentration,kontorovich2008concentration}),
giving an $O(\sqrt{T\log T})$ bound after a union bound over coordinates.
\end{proof}

\subsection{Regret bound}

\begin{theorem}
\label{thm:mainMarkov}
Under Assumptions~\ref{cvx} and \ref{bddness}, for
$\eta_{\theta,t}\le \sqrt{\frac{2\ln 2}{B^2 t}}$ and
$\eta_{x,t} = \frac{D}{G\sqrt{t}}$,
the expected \emph{min--max} static regret of Algorithm~\ref{alg:main}
under Markovian inputs satisfies
\[
\bar R_\cA(T)
=
O(\sqrt{T}) + O(\tau_{\mathrm{mix}}).
\]
\end{theorem}

\begin{proof}
The bounds on $\bbE\{R_1\}$ and $\bbE\{R_2\}$ are unchanged.
For $R_3$, as in the Martingale case,
\[
R_3
\le
\sum_{t=1}^T (\theta_t-\theta^\star)^\top \lambda_t(x^\star),
\]
where $(x^\star,\theta^\star)$ solves
$\min_x \max_\theta \theta^\top\mu(x)$.

Taking conditional expectation,
\[
\mathbb E\!\left[
(\theta_t-\theta^\star)^\top \lambda_t(x^\star)
\mid \mathcal F_{t-1}
\right]
=
(\theta_t-\theta^\star)^\top
\mathbb E[\lambda_t(x^\star)\mid \mathcal F_{t-1}].
\]
Uniform ergodicity implies
\[
\left\|
\mathbb E[\lambda_t(x^\star)\mid \mathcal F_{t-1}] - \mu(x^\star)
\right\|_\infty
\le O(e^{-t/\tau_{\mathrm{mix}}}).
\]
Since $(\theta_t-\theta^\star)^\top\mu(x^\star)\le 0$,
summing over $t$ and taking expectations yields
\[
\bbE\{R_3\} \le O(\tau_{\mathrm{mix}}).
\]
\end{proof}

Combining Lemma~\ref{lem:markov_benchmark_gap} and
Theorem~\ref{thm:mainMarkov}, the expected regret of Algorithm~\ref{alg:main}
with respect to the true benchmark $\bbE\{C_{\opt}\}$ is
\[
O(\sqrt{T\log T}) + O(\tau_{\mathrm{mix}}).
\]



==> R3BoundAdversarial.tex <==

\section{Bounding $R_3$ with the adversarial input}\label{R3ubad}
In this section, we show the best bound one can obtain for $R_3$ on a sample path basis for Algorithm \ref{alg:main} with the 
adversarial input is $O(\eta_\theta T^2)$.

%To prove Lemma \ref{lem:R3} we prove the following Theorem \ref{thm:r3bound}.% which implies Lemma \ref{lem:R3} by choosing $\eta_{\theta,t}=\frac{1}{2B^2\sqrt{t}}$

\begin{theorem}\label{thm:r3bound}
Under Assumption \ref{cvx}, i.e., $\|\lambda_t(x)\|_\infty \le B$, $R_3 \le 2B^2 T \sum_{t=1}^T \eta_{\theta,t} $. %\sum_{t=1}^T\eta_{\theta,t} $.
\end{theorem}
Recall the definitions $\lambda_t(x) = (f_t(x), g_t(x))$,
\[
R_3 \;=\; \min_{x\in\mathcal X}\sum_{t=1}^T \langle\theta_t,\lambda_t(x)\rangle -C_\opt,
\qquad \text{and} \qquad
C_\opt = \min_{x\in\mathcal X}\max_{\theta\in\Delta_2}\sum_{t=1}^T \langle\theta,\lambda_t(x)\rangle.
\]
Thus, an almost natural way (or really the only way for Algorithm \ref{alg:main} that combines OGD+{\it Hedge}) to bound $R_3$ is via exploiting the stability $\sum_t\|\theta_{t+1}-\theta_t\|_1$ of the {\it Hedge} algorithm. Following this path, we next derive  Lemma \ref{lem:L1}, Lemma \ref{lem:telescope} and Lemma \ref{lem:kl} which when combined imply Theorem \ref{thm:r3bound}.


However, it is not sufficient since by substituting $\eta_{\theta,t} = \frac{1}{\sqrt{T}}$  for all $t$, the usual {\it Hedge} step size, we get $R_3= \Omega(T^{3/2})$.


%Proof of Theorem \ref{thm:r3bound} follows by combining Lemma \ref{lem:L1}, Lemma \ref{lem:telescope} and Lemma \ref{lem:kl} that are proved next. 



\begin{lemma}\label{lem:L1} Define the time-averaged vector
$\bar\theta := \frac{1}{T}\sum_{t=1}^T \theta_t \in \Delta_2.$ Then, 

$$R_3 \le B\sum_{t=1}^T \|\theta_t-\bar\theta\|_1.$$
\end{lemma}
\begin{proof}
%\paragraph{Proof that \(R_3 \le \min_x \sum_t \langle\theta_t-\bar\theta,\lambda_t(x)\rangle\).}
%Recall the definitions
%\[
%R_3 \;=\; \min_{x\in\mathcal X}\sum_{t=1}^T \langle\theta_t,\lambda_t(x)\rangle -C_\opt,
%\qquad
%V^\star = \min_{x\in\mathcal X}\max_{\theta\in\Delta_2}\sum_{t=1}^T \langle\theta,\lambda_t(x)\rangle.
%\]

Since \(\bar\theta\) is a particular (constant) element of \(\Delta_2\), for every \(x\in\mathcal X\)
\[
\sum_{t=1}^T \langle\bar\theta,\lambda_t(x)\rangle \le
\max_{\theta\in\Delta_2}\sum_{t=1}^T \langle\theta,\lambda_t(x)\rangle,
\]
and therefore taking the minimum over \(x\) yields
\[
\min_{x\in\mathcal X}\sum_{t=1}^T \langle\bar\theta,\lambda_t(x)\rangle \le C_\opt.
\]
Thus, \[
\begin{aligned}
R_3
&= \min_{x}\sum_{t=1}^T \langle\theta_t,\lambda_t(x)\rangle -C_\opt \\
&\le \min_{x}\sum_{t=1}^T \langle\theta_t,\lambda_t(x)\rangle - \min_{x}\sum_{t=1}^T \langle\bar\theta,\lambda_t(x)\rangle \\
&\le \max_{x}\sum_{t=1}^T \big\langle\theta_t-\bar\theta,\lambda_t(x)\big\rangle,
\end{aligned}
\]
where the last inequality follows as below. 
\\
\newline \noindent
Let $x^\star$ satisfy $u(x^\star)=\min_x u(x)$. 
Then
\[
\min_x u(x)-\min_x v(x)=u(x^\star)-\min_x v(x)\le u(x^\star)-v(x^\star)\le\max_x (u(x)-v(x)),
\]
which proves the claim.

%where the last line uses that subtracting the same quantity from two minima is majorized by taking the minimum of the difference (equivalently, for all functions \(u(x),v(x)\), \(\min_x u(x)-\min_x v(x)\le\min_x(u(x)-v(x))\)).

This proves
\begin{equation}\label{eq:stable1}
R_3 \le \max_{x\in\mathcal X}\sum_{t=1}^T \langle\theta_t-\bar\theta,\lambda_t(x)\rangle.
\end{equation}

Since we are in the bounded setting, for all rounds $t$ and all $x\in\mathcal X$ we have
$\|\lambda_t(x)\|_\infty \le B$. 
%Recall
%\[
%R_3 \;=\; \min_{x\in\mathcal X}\sum_{t=1}^T \langle\theta_t,\lambda_t(x)\rangle -C_\opt
%\le \min_{x\in\mathcal X}\sum_{t=1}^T \langle\theta_t-\bar\theta,\lambda_t(x)\rangle,
%\]
%where $\bar\theta=\tfrac{1}{T}\sum_{t=1}^T\theta_t$. 
Thus, appyling the Hölder's inequality (using duality of $||.||_1$ and $||.||_\infty$ norms) on \eqref{eq:stable1},
\[
\sum_{t=1}^T \langle\theta_t-\bar\theta,\lambda_t(x)\rangle
\le \sum_{t=1}^T \|\theta_t-\bar\theta\|_1 \,\|\lambda_t(x)\|_\infty
\le B\sum_{t=1}^T \|\theta_t-\bar\theta\|_1.
\]
%Taking the minimum over $x$ on the left-hand side cannot increase the right-hand side, hence
Thus,
\[
R_3 \le B\sum_{t=1}^T \|\theta_t-\bar\theta\|_1.
\]
This is the desired inequality.
\end{proof}




Next, we state an elementary inequality without proof.
\begin{lemma}[Deviation from average via consecutive differences]
\label{lem:telescope}
Let $\theta_1,\dots,\theta_T\in\mathbb{R}^d$ be vectors, and define the average
\[
\bar\theta = \frac{1}{T}\sum_{t=1}^T \theta_t.
\]
Then
\[
\sum_{t=1}^T \|\theta_t-\bar\theta\|_1 \;\le\; 2 T\sum_{t=1}^{T-1}\|\theta_{t+1}-\theta_t\|_1.
\]
\end{lemma}

%\begin{proof}
%We first expand the deviation from the average in terms of pairwise distances:
%\[
%\sum_{t=1}^T \|\theta_t-\bar\theta\|_1
%= \frac{1}{T}\sum_{t=1}^T \left\|\sum_{s=1}^T(\theta_t-\theta_s)\right\|_1
%\le \frac{1}{T}\sum_{t=1}^T \sum_{s=1}^T \|\theta_t-\theta_s\|_1.
%\]
%
%Now fix $t<s$. By the triangle inequality,
%\[
%\|\theta_t-\theta_s\|_1 \;\le\;
%\sum_{u=t}^{s-1} \|\theta_{u+1}-\theta_u\|_1.
%\]
%The same bound holds for $s<t$ by symmetry. Inserting \((2)\) into \((1)\) gives
%\[
%\sum_{t=1}^T \|\theta_t-\bar\theta\|_1
%\;\le\; \frac{1}{T}\sum_{t=1}^T\sum_{s=1}^T
%\sum_{u=\min(t,s)}^{\max(t,s)-1} \|\theta_{u+1}-\theta_u\|_1.
%\]
%
%Change the order of summation. For each $u\in\{1,\dots,T-1\}$, the term
%$\|\theta_{u+1}-\theta_u\|_1$ appears once for each ordered pair $(t,s)$
%with $\min(t,s)\le u < \max(t,s)$. The number of such pairs is
%$2(T-u)$. Therefore
%\[
%\sum_{t=1}^T \|\theta_t-\bar\theta\|_1
%\;\le\; \frac{1}{T}\sum_{u=1}^{T-1} 2(T-u)\,\|\theta_{u+1}-\theta_u\|_1.
%\]
%
%Finally, $(T-u)/T \le 1$, hence
%\[
%\sum_{t=1}^T \|\theta_t-\bar\theta\|_1
%\;\le\; 2\sum_{u=1}^{T-1}\|\theta_{u+1}-\theta_u\|_1,
%\]
%which proves the claim.
%\end{proof}

\bigskip

\begin{lemma}[One-step TV bound for Hedge]
\label{lem:kl}
Let \(\{\theta_t\}\) be the Hedge distributions updated by
\[
\theta_{t+1,i} \;=\; \frac{\theta_{t,i}\,e^{\eta_{\theta,t} \lambda_{t,i}}}
{\sum_{j}\theta_{t,j}\,e^{\eta_{\theta,t} \lambda_{t,j}}},
\qquad i=1,\dots,n,
\]
with learning rate \(\eta_{\theta,t}>0\).  Assume the losses satisfy
\(\lambda_{t,i}\in[0,B]\) for all \(i\). Then
\[
\|\theta_{t+1}-\theta_t\|_1 \le \eta_{\theta,t} B.
\]
%More generally, if \(\lambda_{t,i}\in[a,b]\), then
%\(\|\theta_{t+1}-\theta_t\|_1 \le \dfrac{\eta_{\theta,t}(b-a)}{2}\).
\end{lemma}

\begin{proof}



Let
\[
Z_t := \sum_{j}\theta_{t,j} e^{\eta_{\theta,t} \lambda_{t,j}} \;=\; \mathbb{E}_{i\sim\theta_t}\!\big[e^{\eta_{\theta,t} \lambda_{t,i}}\big].
\]
By the definition of Kullback–Leibler divergence,
\[
\begin{aligned}
D_{\mathrm{KL}}(\theta_t\|\theta_{t+1})
&= \sum_i \theta_{t,i} \ln\frac{\theta_{t,i}}{\theta_{t+1,i}}
= \sum_i \theta_{t,i} \ln\frac{\theta_{t,i}}{\theta_{t,i} e^{\eta_{\theta,t} \lambda_{t,i}}/Z_t} \\
&= \sum_i \theta_{t,i} (\ln Z_t - \eta_{\theta,t} \lambda_{t,i})
= \ln Z_t - \eta_{\theta,t}\,\mathbb{E}_{i\sim\theta_t}[\lambda_{t,i}].
\end{aligned}
\]

Let \(\mu := \mathbb{E}_{i\sim\theta_t}[\lambda_{t,i}]\). Then
\(\ln Z_t = \ln \mathbb{E}_{\theta_t}\big[e^{\eta_{\theta,t} \lambda_{t,i}}\big]
= \eta_{\theta,t}\mu + \ln \mathbb{E}_{\theta_t}\big[e^{\eta_{\theta,t}(\lambda_{t,i}-\mu)}\big]\),
so (1) is equivalently
\begin{equation}\label{eq:kl}
D_{\mathrm{KL}}(\theta_t\|\theta_{t+1})
= \ln \mathbb{E}_{\theta_t}\big[e^{\eta_{\theta,t}(\lambda_{t,i}-\mu)}\big].
\end{equation}


Thus to upper bound the one-step KL it suffices to bound the centered MGF
\(\ln \mathbb{E}[e^{\eta_{\theta,t}(\lambda_{t,i}-\mu)}]\).

%\paragraph{Step 2: Hoeffding's mgf bound (proof).}
\begin{proposition}[Hoeffding's MGF bound] For a random variable \(X\) that 
satisfies \(X\in[a,b]\) almost surely and \(\mathbb{E}[X]=\mu\), then for any \(s\in\mathbb R\)
\begin{equation}\label{eq:conc}
\ln\mathbb{E}[e^{s(X-\mu)}] \le \frac{s^2(b-a)^2}{8}.
\end{equation}
\end{proposition}

%\emph{Proof of (H).} Define the function
%\(\psi(s) := \ln\mathbb{E}[e^{s(X-\mu)}]\). Then \(\psi(0)=0\) and
%\(\psi'(s)=\mathbb{E}_{Q_s}[X-\mu]\) where \(Q_s\) is the tilted probability
%measure with density proportional to \(e^{s(X-\mu)}\). The second derivative
%is
%\[
%\psi''(s) = \operatorname{Var}_{Q_s}(X).
%\]
%But \(Q_s\) is still supported inside \([a,b]\), so for any distribution supported on \([a,b]\) the variance is bounded by \((b-a)^2/4\) (indeed the maximum variance on \([a,b]\) is attained by the two-point distribution with mass \(1/2\) at \(a\) and \(b\)). Therefore
%\(\psi''(s) \le (b-a)^2/4\) for all \(s\). Integrating twice from \(0\) to \(s\) and using \(\psi(0)=\psi'(0)=0\) gives
%\[
%\psi(s) \;=\; \int_0^s (s-u)\psi''(u)\,du \;\le\; \int_0^s (s-u)\,\frac{(b-a)^2}{4}\,du
%= \frac{s^2(b-a)^2}{8},
%\]
%which proves (H). \(\square\)

Since \(\lambda_{t,i}\in[0,B]\), using \eqref{eq:conc} in \eqref{eq:kl} with \(X=\lambda_{t,i}\), \([a,b]=[-B,B]\), \(s=\eta_{\theta,t}\), and mean \(\mu\), we get
%\[
%\ln \mathbb{E}_{\theta_t}\big[e^{\eta_{\theta,t}(\lambda_{t,i}-\mu)}\big] \le \frac{\eta_{\theta,t}^2 B^2}{8}.
%\]
%R_3ombining with (2) gives the one-step KL bound
\begin{equation}\label{eq:finalkl}
D_{\mathrm{KL}}(\theta_t\|\theta_{t+1}) \le \frac{\eta_{\theta,t}^2 4B^2}{8}.
\end{equation}

\begin{proposition} [Pinsker's inequality  \cite{bookCover}] For any two probability vectors \(p,q\),
\begin{equation}\label{eq:pinsker}
\|p-q\|_1 \le \sqrt{2\,D_{\mathrm{KL}}(p\|q)}.
\end{equation}
\end{proposition}
Since both $\theta_t$ and $\theta_{t+1}$ are distributions, applying \eqref{eq:pinsker} on \eqref{eq:finalkl}, we get
\[
\|\theta_{t+1}-\theta_t\|_1 \le \sqrt{2\cdot \frac{\eta_{\theta,t}^2 B^2}{2}}
= \eta_{\theta,t} B,
\]
the claimed bound. \qedhere

\end{proof}









%\end{document}

